An algorithm for random signed 3-SAT with Intervals

In signed k-SAT problems, one fixes a set M and a set $\mathcal S$ of subsets of M, and is given a formula consisting of a disjunction of m clauses, each of which is a conjunction of k literals. Each literal is of the form "$x \in S$", where $S \in \mathcal S$, and x is one of n variables. For Interval-SAT (iSAT), M is an ordered set and $\mathcal S$ the set of intervals in M. We propose an algorithm for 3-iSAT, and analyze it on uniformly random formulas. The algorithm follows the Unit Clause paradigm, enhanced by a (very limited) backtracking option. Using Wormald's ODE method, we prove that, if $m/n \le 2.3$, with high probability, our algorithm succeeds in finding an assignment of values to the variables satisfying the formula.

==> todo.tex <==
% isat/todo.tex

\section*{TODO}

\begin{minipage}{.65\linewidth}
\begin{enumerate}[\S~1]
\item Done, I guess :) :)
\item Done, I guess :)
\item Done, I guess :)
\item Done, I guess :)
\item 
  \begin{itemize}
  \item Move some stuff into appendix
  \item Review
  \end{itemize}
\item 
  \begin{itemize}
  \item Review; make sure it all fits with previous section
  \item Some todos left on the margin
  \end{itemize}  
\item Review
\item Done :) :)
\end{enumerate}
\end{minipage}%
\begin{minipage}{.332\linewidth}
  \rotatebox{45}{\fbox{THIS LOOKS GOOD!!! :)}}
\end{minipage}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "full.tex"
%%% fill-column: 165
%%% End: 

